Autonomous Constellation Fault Monitoring with Inter-satellite Links: A Rigidity-Based Approach

To address the need for robust positioning, navigation, and timing services in lunar environments, this paper proposes a novel fault detection framework for satellite constellations using inter-satellite ranging (ISR). Traditionally, navigation satellites can depend on a robust network of ground-based stations for fault monitoring. However, due to cost constraints, a comprehensive ground segment on the lunar surface is impractical for lunar constellations. Our approach leverages vertex redundantly rigid graphs to detect faults without relying on precise ephemeris. We model satellite constellations as graphs where satellites are vertices and inter-satellite links are edges. We identify faults through the singular values of the geometric-centered Euclidean distance matrix (GCEDM) of 2-vertex redundantly rigid sub-graphs. The proposed method is validated through simulations of constellations around the Moon, demonstrating its effectiveness in various configurations. This research contributes to the reliable operation of satellite constellations for future lunar exploration missions.

==> sections/4_1_prediction_model.tex <==
\subsection{Test Statistic Distribution Prediction Model}
\label{sec:fault_detection}
As mentioned in Section~\ref{sec:distribution_singular}, the distribution of the test statistics of the non-fault noisy GCEDM can be approximated as a gamma distribution, where its shape parameters are determined by the relative geometry of the satellites. 
To detect faults by checking if $\teststatistic$ exceeds a certain threshold, we are particularly interested in the tails of the distribution of the non-fault case. 
Therefore, our goal is to develop a model $\hat{f}_{\gamma}$ that can predict the parameters of tails of the $\teststatistic$ (e.g., 99.7 percentile value $\teststatisticpercentile{99.7} $), given the ISR noise magnitude $\sigma_w$ and the relative geometry. 

In this paper, we propose to use the first three singular values $\lambda_1, \lambda_2, \lambda_3$ of the GCEDM and the first three columns of the orthogonal matrix $\bm{U}$ of the singular value decomposition $\bm{u}_1, \bm{u}_2, \bm{u}_3 \in \R^{n} (n: \text{number of satellites in the EDM})$ as the input to the model.
These parameters remain almost constant under noise, when $\sigma_w$ is sufficiently small compared to the ranges.
Compared to using the elements of the GCEDM or EDM as the input, this input is invariant to the permutation of the nodes and is more robust to noise in the ranges.
This results in an input dimension of $3(n+1)$, where $n$ is the number of satellites in the EDM. For this paper, we only use EDMs with 6 satellites for fault detection, so the input size is 21.
%
An example of a 2D histogram that shows the mapping between the first three singular values and the 99.7 percentile of the test statistics ($\teststatisticpercentile{99.7}$) is shown in Figure \ref{fig:2dhist_mars}. For fault detection, we need a model that can map the input to these percentile values, but from Figure \ref{fig:2dhist_mars}, we observe that the map is nonlinear.

In this paper, we trained a neural network with 3 fully connected layers (Table \ref{tab:nn_params}) for the predictor
\begin{equation}
    \gamma_{test, 99.7} = \hat{f}_{\gamma}(\bm{z}_{test}), \quad 
    \bm{z}_{test} = \begin{bmatrix}
    \lambda_1, \lambda_2, \lambda_3, \bm{u}_1^{\top}, \bm{u}_2^{\top}, \bm{u}_3^{\top}
    \end{bmatrix} \in \R^{21}
\end{equation}
The training dataset is obtained by simulating the distribution of $\teststatistic$ for 50000 noisy GCEDMs generated from 6 satellite subgraphs in the target constellation.
Note that the training data can be generated by simulation because we assume we know the noise level $\sigma_w$ and the configuration of the constellation beforehand.
The predictor is trained separately for different constellations so that the predictors have good performance for the geometries that appear frequently in each constellation. 
In future work, we plan to investigate developing a more general predictor, so that it can generate outputs for arbitrary noise magnitudes and percentile values and a wider set of geometries.

\begin{figure}[htb!]
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mars/mars_12_6_50000_10000_p99.pdf}
        \subcaption{2D histogram for the Mars constellation case}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/moon12/moon_12_6_50000_10000_p99.pdf}
        \subcaption{2D histogram for the ELFO constellation case}
    \end{subfigure}
    \caption{A 2D histogram showing the map between the first three singular values of the GCEDM ($\lambda_1, \lambda_2, \lambda_3$, x-axes) and the 99.7 percentile (y axes). The values were sampled from a set of noisy EDMs obtained from subgraphs that appear in a Mars and ELFO constellation shown later in Figure \ref{fig:orbit_mars_case} and Figure \ref{fig:orbit_moon_case}. In this paper, we train a 3-layer neural network to obtain the predictor $f^{\gamma}$ that predicts the 99.7 percentile of the test statistics ($\gamma_{test, 99.7}$) from the first three singular values (and the first three columns of the orthogonal matrix $\bm{U}$) of the GCEDM. The predictor is trained separately for the two cases as they have significantly different geometries.}
    \label{fig:2dhist_mars}
\end{figure}

\begin{table}[htb!]
    \centering
    \caption{The configuration of the neural network predictor. The predictor takes in the first three singular values and the elements of its corresponding column vectors and outputs the estimated 99.7 percentile value of the test statistics $\teststatistic$. }
    \begin{tabular}{|c c c c|} \hline
       Layer & Input Size & Output Size & Activation \\ \hline
        1 & 21 & 128 & ReLU \\
        2 & 128 & 32 & ReLU \\
        3 & 32 & 1  & - \\ \hline
    \end{tabular}
    \label{tab:nn_params}
\end{table}


==> sections/old/4_0_simulation.tex <==

\section{Satellite Fault Detection Simulation}
\label{sec:simulation}
% \begin{enumerate}
%     \item Metrics (i.e., TPR)
%     \item Earth / Mars Case
%     \item Moon Case
% \end{enumerate}

\subsection{Simulation Configuration and Evaluation Metrics}
We validate our proposed algorithms for the constellations around the Moon. 
The detailed configurations of the constellations are shown later in each section.
For both simulation cases, the orbits are propagated in the two-body propagator without perturbations.
The visibility of the links is calculated assuming that the links are visible when it is not occulted by the planetary body.

We run 500 Monte-Carlo analyses with randomly sampled initial time (within one orbital period) and a set of fault satellites. 
We tested 60 combinations of different detection and simulation parameters: 3 different numbers of fault satellites (1, 2, or 3), 5 different fault magnitudes ($\bar{b}$ = 5, 8, 10, 15, 20 m), and 4 different detection time intervals $(DI = 1, 2, 3, 5)$. 
The timestep between each detection for $DI \geq 2$ is set to 60 seconds. 
For the other hyper-parameters, we used $k=6, \delta_{nf} = 10, \delta_{rf} = 0.2$.
Note that the seed of the Monte-Carlo simulation is fixed so that the performance for different parameters is compared among the same conditions except the parameters. 

We compute the following metrics to evaluate the performance of the detection algorithm
\begin{align}
    \text{True Positive Rate} \ (TPR) &= \frac{TP}{TP + FN} \\
    \text{False Positive Rate} \ (FPR) &= \frac{FP}{FP + TN} \\
    \text{Positive Predictive Value} \ (PPV) &=  \frac{TP}{TP + FP} \\
    \text{F1 value} \ (F1) &= \frac{2 \times PPV \times TPR}{PPV + TPR} 
\end{align}
where $TP, FN, FP, TN$ is the total number of true positives (fault satellite detected as fault), false negatives (fault satellite detected as non-fault), false positives (non-fault satellite detected as fault), and true negatives (non-fault satellite detected as non-fault). 




==> sections/old/4_1_mars_case.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Mars case
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Case 1: Mars Walker Constellation}
\label{sec:mars_sim}
The first example is the Walker Delta constellation around Mars, with a total of 12 satellites equally spread to 4 different orbital planes. The orbital elements of the constellation are shown in Table \ref{tab:mars_constellation}. The constellation and the links at $t=0$ are shown in Figure \ref{fig:mars_orbit}. The number of 6-cliques in the constellation with the number of subgraphs containing satellite 1,2,3 (satellites in the first plane) is shown in Figure \ref{fig:mars_nclique}. For all timesteps, each satellite has at least 32 participations within a 6-clique that can be used for fault detection.

\begin{table}[H]
    \centering
    \caption{Orbital elements of the Mars Walker-Delta constellation (Case 1)}
    \begin{tabular}{|c|c c c c c c|}  \hline
       Plane & Semi-Major Axis & Eccentricity & Inclination  & RAAN &  Argument of Periapsis & 
       Mean Anomaly  \\
       &  $a$ [km] & $e$ []  & $i$ [deg] & $\Omega$ [deg] & $\omega$ [deg]  & $M$ [deg]       \\ \hline
       1 &  15850.55 & 0.0 & 60 &  0 & 0 & [0, 120, 240 ] \\
       2 &  15850.55 & 0.0 & 60 &  90 & 0 & [114.6, 234.6, 354.6] \\
       3 &  15850.55 & 0.0 & 60 &  180 & 0 & [229.2, 349.2, 109.2] \\ 
       4 &  15850.55 & 0.0 & 60 &  -90 & 0 & [343.8, 103.8, 223.8] \\  \hline
    \end{tabular}
    \label{tab:mars_constellation}
\end{table}

The fault detection results compared to the fixed threshold predictor are shown in Figure \ref{fig:comparison_mars}. For the fixed threshold predictor, $\teststatisticpercentile{99.7}$ was fixed to the 99.7 percentile value of the test statistics, which was computed from 50000 non-fault subgraphs that were randomly sampled from the entire simulation window. 
We observe that compared to the fixed threshold predictor, the machine learning predictor has a higher TPR, especially at lower fault magnitudes. 
This is because the predicted $\gamma_{test, 99.7}$ is less conservative compared to the fixed threshold, and considers more satellites (subgraphs) as fault candidates. 
However, the neural network predictor also has a higher FPR than the fixed threshold. This is because since the fixed threshold predictor is conservative, it only considers subgraphs of which the singular values and singular vectors of GCEDMs are largely perturbed, which is likely to be fault satellites. 
If it desired to make the FPR lower for the neural network predictor, we can do so by increasing the hyperparameter $\delta_{nf}$ and $\delta_{rf}$.

The sensitivity of fault magnitude, detection timesteps, and the number of faults to the detection metrics are shown in Figure \ref{fig:plot3_mars_case}. 
In general, the true positive rate is higher and the false positive rate is lower if we have a larger false magnitude and a smaller number of fault satellites, as it would be easier to detect fault subgraphs and distinguish which is the fault satellite. 
Increasing the detection time interval (DI) increases both the true positive rate and the false positive rate. Therefore, detection length can be used as a hyper-parameter to balance the true positive rate and false positive rate.

\begin{figure}[tb!]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/orbits/mars_12.pdf}
        \subcaption{Orbital planes with satellite position (black points) and links (orange line) at the initial time epoch. The orbital period is half of Mars's solar day. The high altitude reduces occultation and enables a dense communication topology.}
        \label{fig:mars_orbit}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mars/exp_mars_nsat_12_e_0_p_4_f_2_nrev_2_ideg_60_tsim_44321.22_s_ncliques6.pdf}
        \subcaption{Transition of the number of 6-cliques over one orbital period. Each satellite has at least 32 of 6 cliques that contain itself throughout the orbit.}
        \label{fig:mars_nclique}
    \end{subfigure}
    \caption{Case 1: Walker-Delta constellation around Mars with 12 satellites }
    \label{fig:orbit_mars_case}
\end{figure}

% Results (Comparison)
\begin{figure}[tb!]
    \centering
    \includegraphics[width=\linewidth]{figures/mars/metrics_nz3_nmc_500_nfm_5_nfs_3_ndt_4_predictor_comparison.pdf}
    \caption{Case 1 (Mars constellation): The detection results for different fault magnitudes and the detection time interval (DI). The number of faults is fixed to one. The detector using the fixed threshold is shown in a dashed line, while the detector using the trained neural network is shown in a solid line. The neural network predictor has a higher true positive rate at the cost of having a higher false positive rate since it adaptively changes the threshold and considers more satellites as fault candidates. The fixed threshold is conservative since it is based on the singular value distribution over all subgraphs throughout the orbits. }
    \label{fig:comparison_mars}
\end{figure}

% Results (3D Plots)
\begin{figure}[tb!]
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mars/plot3_nz3_nmc_500_nfm_5_nfs_3_ndt_4_predictor_False.pdf}
        \subcaption{Detection results with fixed threshold}
        \label{fig:plot3_mars_fixed}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/mars/plot3_nz3_nmc_500_nfm_5_nfs_3_ndt_4_predictor_True.pdf}
        \subcaption{Detection results with neural network predictor}
        \label{fig:plot3_mars_nn}
    \end{subfigure}
    \caption{Case 1 (Mars constellation): Detection results (z-axis) shown as a 3D plot for different fault magnitudes (x-axis), number of detection timesteps (y-axis), and number of faults (planes). The true positive rate decreases with a larger number of faults, since when we have multiple fault satellites that have many shared subgraphs, the first round (satellite removal) of the greedy algorithm can remove the majority of the subgraphs containing the second (and third) false satellite as well, making it difficult to detect the remaining fault satellites. Also, a larger number of faults leads to larger false positive rates, as the 4th singular vector of the GCEDM becomes more perturbed. }
    \label{fig:plot3_mars_case}
\end{figure}

==> sections/old/4_2_moon_case.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Moon case
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Case 2: Elliptical Lunar Frozen Orbit Constellation}
\label{sec:moon_sim}
The second simulation scenario is the Elliptical Lunar Frozen Orbit (ELFO) constellation with a total of 12 satellites equally spread to 4 different orbital planes. The orbital elements of the constellation are shown in Table \ref{tab:moon_constellation}. The constellation and the links at $t=0$ are shown in Figure \ref{fig:moon_orbit}. The number of 6-cliques in the constellation with the number of subgraphs containing satellite 1,2,3 (satellites in the first plane) is shown in Figure \ref{fig:moon_nclique}. In this scenario, each satellite experiences a time window where they have zero or few self-containing subgraphs, where faults cannot be detected.

\begin{table}[H]
    \centering
    \caption{Orbital elements of the ELFO constellation (Case 2)}
    \begin{tabular}{|c|c c c c c c|}  \hline
       Plane & Semi-Major Axis & Eccentricity & Inclination  & RAAN &  Argument of Periapsis & 
       Mean Anomaly  \\
       &  $a$ [km] & $e$ []  & $i$ [deg] & $\Omega$ [deg] & $\omega$ [deg]  & $M$ [deg]       \\ \hline
       1 &  6142.4 & 0.6 & 57.7 &  -90 & 90 & [0, 120, 240] \\
       2 &  6142.4 & 0.6 & 57.7 &  0 & 90 & [30, 150, 270] \\
       3 &  6142.4 & 0.6 & 57.7 &  90 & 90 & [60, 180, 300] \\ 
       4 &  6142.4 & 0.6 & 57.7 &  180 & 90 & [90, 210, 330] \\  \hline
    \end{tabular}
    \label{tab:moon_constellation}
\end{table}

The fault detection results compared to the fixed threshold predictor are shown in Figure \ref{fig:comparison_moon}, and the sensitivity of fault magnitude, detection timesteps, and the number of faults to the detection metrics are shown in Figure \ref{fig:plot3_moon_case}. In general, the observed relationship between the parameters and the detection metrics is the same as in the Mars case. However, the TPR is capped around 0.92, because at any time there will be 1 satellite (8.3$\%$ of 12) located near the perilune, whose fault cannot be detected because of the limited number of self-containing subgraphs.

\begin{figure}[tb!]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/moon12/exp_moon_nsat_12_p_4_nrev_80_tsim_43198.12492069844_s_constellation.pdf}
        \subcaption{Orbital planes with satellite position (black points) and links (orange line) at the initial time epoch. Satellites near the perilune have only 4 or 5 links available due to occultation by the Moon. }
        \label{fig:moon_orbit}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/moon12/exp_moon_nsat_12_p_4_nrev_80_tsim_43198.12492069844_s_ncliques6.pdf}
        \subcaption{Number of 6-cliques for different time epochs. The satellite near the perilune has few or zero 6-cliques containing itself due to the occultation by the Moon.}
        \label{fig:moon_nclique}
    \end{subfigure}
    \caption{Case 2: ELFO constellation around Moon with 12 satellites. }
    \label{fig:orbit_moon_case}
\end{figure}

% Results (Comparison)
\begin{figure}[htb!]
    \centering
    \includegraphics[width=\linewidth]{figures/moon12/metrics_nz3_nmc_500_nfm_5_nfs_3_ndt_4_predictor_comparison.pdf}
    \caption{Case 2 (ELFO constellation): The detection results for different fault magnitudes and the detection length (DL). The number of faults is fixed to one. The detector using the fixed threshold is shown in a dashed line, while the detector using the trained neural network is shown in a solid line. }
    \label{fig:comparison_moon}
\end{figure}

% Results (3D Plots)
\begin{figure}[tb!]
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/moon12/plot3_nz3_nmc_500_nfm_5_nfs_3_ndt_4_predictor_False.pdf}
        \subcaption{Detection results with fixed threshold}
        \label{fig:moon_fixed_result}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/moon12/plot3_nz3_nmc_500_nfm_5_nfs_3_ndt_4_predictor_True.pdf}
        \subcaption{Detection results with neural network predictor}
        \label{fig:moon_nn_result}
    \end{subfigure}
    \caption{Case 2 (ELFO constellation): Detection results (z-axis) shown as a 3D plot for different fault magnitudes (x-axis), number of detection timesteps (y-axis), and number of faults (planes).  }
    \label{fig:plot3_moon_case}
\end{figure}


%% Table
\begin{table}[ht!]
\centering
\caption{Fault detection result for different number of faults, fault magnitude, fault detection threshold, and detection length (DL). The best TPR, FPR, and P4 values for each (number of faults, fault magnitude) pair are highlighted in blue. In general, TPR improves as the threshold decreases and detection length increases, and FPR improves as the threshold increases and detection length decreases. The P4 values are maximized at higher thresholds and longer DL at smaller fault magnitudes, and vice versa for larger fault magnitudes.  }
\begin{tabular}{Ic|c|cI  c|c|cI  c|c|cI  c|c|cI}
\bhline{1pt}
\multirow{3}{*}{Faults} & \multirow{2}{*}{Thresh} & \multirow{2}{*}{DL} & \multicolumn{3}{cI}{True Positive Rate} & \multicolumn{3}{cI}{False Positive Rate} & \multicolumn{3}{cI}{P4 value} \\
 &  &  & \multicolumn{3}{cI}{Fault Magnitude [m]} & \multicolumn{3}{cI}{Fault Magnitude [m]} & \multicolumn{3}{cI}{Fault Magnitude [m]} \\
 & [$\%$] & [] & 5 & 10 & 20 & 5 & 10 & 20 & 5 & 10 & 20 \\
\bhline{1pt}
\multirow{12}{*}{1} & \multirow{4}{*}{99.9} & 1  & 0.006 & 0.374 & 0.864 & \color{blue}{ \textbf{ 0.001 } } & \color{blue}{ \textbf{ 0.000 } } & \color{blue}{ \textbf{ 0.001 } } & 0.023 & 0.698 & 0.955 \\
 &  & 2 & 0.042 & 0.582 & 0.896 & 0.001 & 0.002 & 0.002 & 0.147 & 0.833 & 0.964 \\
 &  & 3 & 0.048 & 0.742 & 0.908 & 0.002 & 0.002 & \color{blue}{ \textbf{ 0.001 } } & 0.165 & 0.908 & \color{blue}{ \textbf{ 0.969 } } \\
 &  & 5 & 0.124 & 0.854 & 0.918 & 0.005 & 0.001 & 0.003 & 0.345 & \color{blue}{ \textbf{ 0.951 } } & 0.968 \\
\cline{2-12}
 & \multirow{4}{*}{99} & 1  & 0.146 & 0.776 & 0.900 & 0.015 & 0.005 & 0.006 & 0.362 & 0.911 & 0.952 \\
 &  & 2 & 0.450 & 0.866 & 0.914 & 0.023 & 0.014 & 0.013 & 0.682 & 0.917 & 0.936 \\
 &  & 3 & 0.530 & 0.874 & 0.924 & 0.032 & 0.026 & 0.019 & 0.712 & 0.888 & 0.922 \\
 &  & 5 & 0.744 & 0.892 & \color{blue}{ \textbf{ 0.926 } } & 0.050 & 0.041 & 0.039 & \color{blue}{ \textbf{ 0.774 } } & 0.854 & 0.871 \\
\cline{2-12}
 & \multirow{4}{*}{95} & 1  & 0.478 & 0.866 & 0.908 & 0.055 & 0.039 & 0.037 & 0.618 & 0.852 & 0.870 \\
 &  & 2 & 0.712 & 0.896 & 0.922 & 0.076 & 0.069 & 0.075 & 0.703 & 0.792 & 0.790 \\
 &  & 3 & 0.758 & 0.888 & 0.918 & 0.098 & 0.096 & 0.098 & 0.681 & 0.736 & 0.743 \\
 &  & 5 & \color{blue}{ \textbf{ 0.808 } } & \color{blue}{ \textbf{ 0.906 } } & 0.922 & 0.108 & 0.115 & 0.116 & 0.685 & 0.709 & 0.713 \\
\cline{2-12}
\bhline{1pt}
\multirow{12}{*}{2} & \multirow{4}{*}{99.9} & 1  & 0.109 & 0.328 & 0.813 & \color{blue}{ \textbf{ 0.004 } } & 0.025 & 0.005 & 0.319 & 0.606 & 0.929 \\
 &  & 2 & 0.173 & 0.458 & 0.853 & 0.007 & 0.026 & 0.005 & 0.436 & 0.714 & 0.944 \\
 &  & 3 & 0.216 & 0.515 & 0.863 & 0.009 & 0.027 & 0.007 & 0.500 & 0.750 & 0.945 \\
 &  & 5 & 0.250 & 0.608 & 0.884 & 0.018 & 0.033 & \color{blue}{ \textbf{ 0.005 } } & 0.531 & 0.795 & \color{blue}{ \textbf{ 0.956 } } \\
\cline{2-12}
 & \multirow{4}{*}{99} & 1  & 0.246 & 0.603 & 0.854 & 0.022 & \color{blue}{ \textbf{ 0.022 } } & 0.009 & 0.521 & 0.810 & 0.939 \\
 &  & 2 & 0.376 & 0.721 & 0.875 & 0.030 & 0.028 & 0.010 & 0.643 & 0.857 & 0.944 \\
 &  & 3 & 0.439 & 0.774 & 0.880 & 0.045 & 0.027 & 0.015 & 0.672 & \color{blue}{ \textbf{ 0.881 } } & 0.938 \\
 &  & 5 & 0.537 & 0.802 & \color{blue}{ \textbf{ 0.896 } } & 0.060 & 0.038 & 0.020 & 0.716 & 0.877 & 0.937 \\
\cline{2-12}
 & \multirow{4}{*}{95} & 1  & 0.417 & 0.775 & 0.865 & 0.055 & 0.032 & 0.023 & 0.641 & 0.874 & 0.921 \\
 &  & 2 & 0.581 & 0.815 & 0.875 & 0.071 & 0.056 & 0.045 & 0.727 & 0.856 & 0.894 \\
 &  & 3 & 0.627 & 0.841 & 0.885 & 0.090 & 0.067 & 0.066 & \color{blue}{ \textbf{ 0.729 } } & 0.852 & 0.870 \\
 &  & 5 & \color{blue}{ \textbf{ 0.664 } } & \color{blue}{ \textbf{ 0.850 } } & 0.886 & 0.106 & 0.093 & 0.090 & 0.728 & 0.823 & 0.840 \\
\cline{2-12}
\bhline{1pt}
\multirow{12}{*}{3} & \multirow{4}{*}{99.9} & 1  & 0.161 & 0.277 & 0.620 & \color{blue}{ \textbf{ 0.010 } } & \color{blue}{ \textbf{ 0.050 } } & \color{blue}{ \textbf{ 0.043 } } & 0.414 & 0.537 & 0.800 \\
 &  & 2 & 0.197 & 0.338 & 0.659 & 0.018 & 0.060 & 0.046 & 0.463 & 0.589 & 0.817 \\
 &  & 3 & 0.214 & 0.379 & 0.685 & 0.024 & 0.063 & 0.046 & 0.482 & 0.622 & 0.830 \\
 &  & 5 & 0.257 & 0.410 & 0.713 & 0.030 & 0.078 & 0.048 & 0.531 & 0.634 & 0.841 \\
\cline{2-12}
 & \multirow{4}{*}{99} & 1  & 0.233 & 0.428 & 0.675 & 0.032 & 0.055 & 0.047 & 0.501 & 0.669 & 0.824 \\
 &  & 2 & 0.297 & 0.513 & 0.721 & 0.054 & 0.066 & 0.045 & 0.554 & 0.717 & 0.848 \\
 &  & 3 & 0.330 & 0.566 & 0.732 & 0.068 & 0.068 & 0.049 & 0.574 & 0.747 & \color{blue}{ \textbf{ 0.849 } } \\
 &  & 5 & 0.399 & 0.597 & \color{blue}{ \textbf{ 0.739 } } & 0.078 & 0.075 & 0.052 & 0.626 & 0.758 & 0.849 \\
\cline{2-12}
 & \multirow{4}{*}{95} & 1  & 0.337 & 0.572 & 0.689 & 0.071 & 0.067 & 0.050 & 0.579 & 0.751 & 0.828 \\
 &  & 2 & 0.409 & 0.625 & 0.725 & 0.101 & 0.074 & 0.052 & 0.614 & 0.774 & 0.843 \\
 &  & 3 & 0.459 & \color{blue}{ \textbf{ 0.672 } } & 0.734 & 0.107 & 0.074 & 0.061 & 0.645 & \color{blue}{ \textbf{ 0.797 } } & 0.838 \\
 &  & 5 & \color{blue}{ \textbf{ 0.497 } } & 0.671 & 0.729 & 0.112 & 0.089 & 0.070 & \color{blue}{ \textbf{ 0.666 } } & 0.783 & 0.828 \\
\cline{2-12}
\bhline{1pt}
\end{tabular}
\label{tab:MoonResult}
\end{table}
 
